Incorporating Voice Instructions in Model-Based Reinforcement Learning for Self-Driving Cars

This paper presents a novel approach that supports natural language voice instructions to guide deep reinforcement learning (DRL) algorithms when training self-driving cars. DRL methods are popular approaches for autonomous vehicle (AV) agents. However, most existing methods are sample- and time-inefficient and lack a natural communication channel with the human expert. In this paper, how new human drivers learn from human coaches motivates us to study new ways of human-in-the-loop learning and a more natural and approachable training interface for the agents. We propose incorporating natural language voice instructions (NLI) in model-based deep reinforcement learning to train self-driving cars. We evaluate the proposed method together with a few state-of-the-art DRL methods in the CARLA simulator. The results show that NLI can help ease the training process and significantly boost the agents' learning speed.

==> test.tex <==
Deep reinforcement learning (DRL) methods are popular approaches for AV. A DRL agent learns by interacting with the driving environment and gradually forms a good policy that satisfies constraints in the  environment. An effective policy can take up many trial-and-error learning experiences. In each learning episode, the agent improves its policy slightly towards an optimization objective, which in most cases is to  maximize the long-term expected cumulative rewards~\citep{rl}.
While these algorithms show promising results, most of them are sample inefficient and require substantial training episodes. 

Model-based reinforcement learning has been proposed to improve sample efficiency by learning an environmental model and using the model to better plan the actions. 

% Niche
However, learning the policy and that of the environmental model is still quite time and sample-consuming.  
When watching an agent's learning curve develop, it is not uncommon for an engineer to have certain words or thoughts come to her mind and almost verbalize to the agent: ``Hey, that move is stupid'', ``Good job!'' or ``Just go there.'' When she sees surprisingly good moves, she would like to let the agent know, and vice versa. However, such a ``direct'', natural, and quick communication channel does not exist.  

On the other hand, we notice that a human novice driver could successfully learn driving with much less training. Human drivers have a human coach giving instructions and evaluative feedback. During a lesson, the student driver does the driving, the coach verbally delivers commands, praises, scolds, and sometimes explains traffic rules and driving conventions paired with stories and reasoning. Their way of communication is natural language (NL) utterances. The student may not speak much while focusing on driving and learning; the coach does most of the talking. Compared to an artificial learner, only a small amount of instructions from the coach is needed by the human student and she learns quite efficiently. On average, a new human driver takes three to five behind-the-wheel classes, each of which lasts around two hours, to pass the road test for a class-D license.\footnote{\url{https://dmv.dc.gov/page/mandatory-driver-education}.}


This motivates us to propose a new way to communicate and train autonomous car agents. In this paper, we propose to give natural language voice instructions to train AV agents directly. Compared to keyboard strokes or other control commands, natural language is a very convenient, natural, and fast communication method. Recent progress in Automated Speech Recognition (ASR), Natural Language Processing (NLP), and personal assistants should have been proliferated to allow people to interact with the learning agents with their voice naturally. Our goal is to provide the agents with the most natural and direct interference and improve and accelerate their learning. 

The voice training interface that we present in this paper can potentially facilitate two scenarios. First, it can help machine learning practitioners interact with their learning algorithms more naturally and directly impact the agent's learning process. Second, the voice inputs allow the non-technical end-user to continue the training after purchasing the agent home. It is like online learning after they  have owned the product for personal use. 

In this paper, we propose incorporating voice instructions in model-based deep reinforcement learning to train self-driving cars. First, we collect voice instructions offline and build a training dataset and a taxonomy of NL instructions. The data analysis shows that most NL instructions are indeed about actions and rewards for the agent. Second, we build a human-in-the-loop model-based DRL framework that can incorporate live voice instructions. Two places in a model-based RL algorithm can incorporate natural language instructions. The first is policy learning, where the natural language instructions can improve or overwrite the agent's actions. The second is the environmental reward model. Ideally, a reward function for the self-driving car would need to handle multiple objectives, such as safety, conforming to traffic rules, speed under control, and passengers feeling comfortable. 
Oftentimes, the reward function is pre-set and hand-crafted by experts before the learning starts, which is not flexible and may not adapt well to the dynamically changing situations while driving. Allowing human interference during training can diversify the reward function from its pre-set formulation and better suit a real-world situation. 
